Stop Reasoning! When Multimodal LLM with Chain-of-Thought Reasoning Meets Adversarial Image

Multimodal LLMs (MLLMs) with a great ability of text and image understanding have received great attention. To achieve better reasoning with MLLMs, Chain-of-Thought (CoT) reasoning has been widely explored, which further promotes MLLMs' explainability by giving intermediate reasoning steps. Despite the strong power demonstrated by MLLMs in multimodal reasoning, recent studies show that MLLMs still suffer from adversarial images. This raises the following open questions: Does CoT also enhance the adversarial robustness of MLLMs? What do the intermediate reasoning steps of CoT entail under adversarial attacks? To answer these questions, we first generalize existing attacks to CoT-based inferences by attacking the two main components, i.e., rationale and answer. We find that CoT indeed improves MLLMs' adversarial robustness against the existing attack methods by leveraging the multi-step reasoning process, but not substantially. Based on our findings, we further propose a novel attack method, termed as stop-reasoning attack, that attacks the model while bypassing the CoT reasoning process. Experiments on three MLLMs and two visual reasoning datasets verify the effectiveness of our proposed method. We show that stop-reasoning attack can result in misled predictions and outperform baseline attacks by a significant margin.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/sec5_anl.tex <==
\subsection{Influence of CoT}

% \subsubsection{How does CoT reasoning influence MLLMs' robustness?}\label{sec:cot-rob}
% % The key information in the rationale makes the attack more difficult.

% % 1. changes in rationale with answer attack -> answer inferring levearage the rationale
% % 2. 

% The extra robustness is attributed to the difficulty of deliberately modifying the rationale part generated by CoT reasoning, because:
% \begin{itemize}
%     \item Changing the rational part generated by CoT reasoning adds additional efforts than only changing the answer part in the prediction that is generated without CoT reasoning.
%     \item Due to the randomness and uncertainly of every rationale content, it is much more difficult to locate precisely on critical information in the rationale part and employ attacks.
% \end{itemize}
% When models infer answers with CoT, the information in the CoT reasoning process is used.



% As shown in Table \ref{tab:ans_att_change}, most samples that were successfully attacked under the answer attack have a changed rationale even if the rationale is not targeted in the attack. 
% The results indicate that compared with models without CoT, to attack a model with CoT, the rationales need to be changed besides the answer, increasing the needed attack effort and leading to the answer attack's ineffectiveness.

% \begin{figure}[t]
% % \vskip 0.2in
% % \begin{subfigure}{\columnwidth}
% % % \vskip 0.2in
% % \centering
% % \includegraphics[width=\columnwidth]{Figure/wo_cot_ch.pdf}
% % \vskip -0.1in
% % \caption{Inference change of answer attack on the model without the CoT process. The changes start from the choice.}
% % \label{fig-wo_chg}
% % \end{subfigure}
% % \vskip -0.2in
% \begin{subfigure}
% \centering
% \includegraphics[width=\columnwidth]{Figure/key_ch.pdf}
% \vskip -0.1in
% \caption{Key Change Example.
% The replication of the answer serves as the key information to infer the answer from the rationale. After the answer attack, the keyword in the rationale is also altered, even though the attack exclusively targets the answer.
% % The replication of the answer is the key information to infer the answer from the rationale. After the answer attack, the keyword is also changed, even though the attack only focuses on the answer.
% }
% \label{fig-ch_key}
% \end{subfigure}
% % \vskip -0.2in
% \begin{subfigure}
% \centering
% \includegraphics[width=\columnwidth]{Figure/trv_ch (1).pdf}
% \vskip -0.1in
% \caption{Trivial Change Example. The replication of the answer is the key information to infer the answer from the rationale. After the answer attack, the keyword is not changed, while the other part of the rationale is changed.}
% \label{fig-ch_trv}
% \end{subfigure}
% % \vskip -0.2in
% \end{figure}

% % This is logical because the model is attacked only based on the choice letter part.



% % \subsubsection{Rationales Are Hard To Be Efficiently Changed}
% % \subsubsection{Why CoT increase MLLMs' robustness under rationale attack?}

% % %%%%%%%%%%%%%%%%%%%%%%%%% GPT %%%%%%%%%%%%%%%%%%%%%%%%%

% To deepen our comprehension, we classified these changes into two categories: key changes and trivial changes. A key change refers to modifications on words crucial for deducing a correct answer, where an example is given in Figure \ref{fig-ch_key}. A trivial change (as illustrated with the example given in Figure \ref{fig-ch_trv}), on the other hand, refers to those modifications on words that are non-crucial for deducing a correct answer while leave key information untouched.
% % For example, only the sentence structure changes, while the semantic information remains similar (refer to Figure \ref{fig-ch_trv}). 

% In the examined testing records, we observed that changes to crucial words are typically straightforward, involving only the modification of specific keywords. Conversely, changes to the non-crucial words appear to be intricate, leading multiple words changed. Note that although altering crucial information (words) in the rationale part appears to be short, precisely identifying the crucial information is hard and modifying them is even more difficult. The main reason is because of the complexity on locating the places where a crucial information can appear as well as understanding the importance of those targeted information. Given this complexity, CoT reasoning coincidentally introduces extra obstacles for the attacker so that the robustness of an MLLM with CoT seems to be enhanced.
%%%%%%%%%%%%%%%%%%%%%%%%%%%END%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%% ORG %%%%%%%%%%%%%%%%%%%%%%%%%
% The rationale in the remaining samples underwent comprehensive alterations.
% For a better understanding, we categorized the changes into two categories: key changes and trivial changes. 
% Key changes refer to alterations in words that are crucial for inferring the answer, such as the replication of the choice content (see Figure \ref{fig-ch_key}). 
% Trivial changes, on the other hand, refer to alterations that are unimportant for inferring the answer, while the keywords remain unchanged.
% For instance, only the sentence structure changes, and the semantic information remains similar (see Figure \ref{fig-ch_trv}).
% After exploring the samples, we found that the changes in keywords are usually simple, i.e., only the keywords are changed, while the changes in the trivial part are usually complex, i.e., several words are changed.
% It seems to be an efficient way to only change the keywords in rationale.
% However, it is hard to locate and change them precisely since they vary their locations in different attack iterations.
% Thus, an efficient attack is hard to perform, further increasing the robustness of MLLMs with CoT.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Even though the keyword located within one inference can be changed, the same keyword can appear in another location in the next inference.
% However, what is interesting is that most samples still have the words ``The answer is'' unchanged (see Figure \ref{fig-ch_key}, \ref{fig-ch_trv}).

% However, the information in the rationale needed for the answer inferring process is hard to locate. Thus, a precise attack is hard to perform, further increasing the robustness of MLLMs with CoT.


% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{Figure/key_ch.pdf}}
% \caption{Key change.
% The replication of the answer serves as the key information to infer the answer from the rationale. After the answer attack, the keyword in the rationale is also altered, even though the attack exclusively targets the answer.
% % The replication of the answer is the key information to infer the answer from the rationale. After the answer attack, the keyword is also changed, even though the attack only focuses on the answer.
% }
% \label{fig-ch_key}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{Figure/trv_ch (1).pdf}}
% \caption{Trivial change. The replication of the answer is the key information to infer the answer from the rationale. After the answer attack, the keyword is not changed, while the other part of the rationale is changed.}
% \label{fig-ch_trv}
% \end{center}
% \vskip -0.2in
% \end{figure}


% \subsubsection{Answer Attack Analysis}\label{sec-ch_ana}
% The answer attack is applicable to models with and without CoT. Models prompted without CoT typically output the answer in the first sentence. Upon examining the samples under attack, we found that changes in samples without CoT appear after the choice, while the other words remain identical to those without attack (see Figure \ref{fig-wo_chg}).



% %%%%%%%%%%%%%%%%%%%%%%%%% GPT %%%%%%%%%%%%%%%%%%%%%%%%%
% However, this is not the case for models employing the CoT reasoning process. 
% From a pool of 80 samples across all datasets and models, only 10 had changes after choice and retained an unchanged rationale. 
% The rationale in the remaining samples underwent comprehensive alterations.

% For a better understanding, we categorized the changes into two categories: key changes and trivial changes. 
% Key changes refer to alterations in words that are crucial for inferring the answer, such as the replication of the choice content (see Figure \ref{fig-ch_key}). 
% Trivial changes, on the other hand, refer to alterations that are unimportant for inferring the answer, while the key words remain unchanged.
% For instance, only the sentence structure changes, and the semantic information remains similar (see Figure \ref{fig-ch_trv}).
% Further analysis was conducted on 40 successfully attacked samples with altered rationales from the A-OKVQA dataset on both models, and the distribution is detailed in Table \ref{tab-ch_chg}.
%%%%%%%%%%%%%%%%%%%%%%%%% ORG %%%%%%%%%%%%%%%%%%%%%%%%%
% But it is not so on the models with CoT. 
% We picked 80 samples across all datasets and models.
% Only 10 of them have an unchanged rationale.
% The rationale in other samples has all changed.
% We observe that with the samples in the A-OKVQA dataset, some words may be treated as the key information to infer the answer from the question, e.g., the replication of the correct choice content.
% So, we divided the changes in the rationale into two categories: key and trivial information (see Figure \ref{fig-ch_key}, Figure \ref{fig-ch_trv}).
% We picked 20 successfully attacked samples with a changed rationale from the A-OKVQA dataset on both models.
% The distribution is shown in Table \ref{tab-ch_chg}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%% GPT %%%%%%%%%%%%%%%%
% The absence of unchanged rationales suggests that the rationale significantly influences the answer. 
% Moreover, the different distributions of the changes in both models show that the specific part of the rationale that exerts the most influence on the answer may vary from one model to another.
% However, a quarter of the changes on OpenFlamingo and almost half of the changes on MiniGPT4 are trivial changes, suggesting that what humans perceive as key information may not necessarily be the most critical part for the model's decision-making process.
%%%%%%%%%%%%%% ORG %%%%%%%%%%%%%%%%%
% When the model leverages the CoT reasoning process, the rationale influences the answer.  
% It is hard to change the answer while keeping the rationale part unchanged.
% But which part of the rationale influences the answer differs from model to model.
% The key information may not be the most important part of the model, although it is crucial for human beings.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{Rationale Attack Analysis}
% %%%%%%%%%%%%%%%% GPT %%%%%%%%%%%%%%%%%%%%%%
% Section \ref{sec-ch_ana} indicates that, in most scenarios, a successful attack on the model necessitates a change in the rationale.
% However, the changes in the rationale part under answer attack scenarios are passive, occurring because the answer needs modification. 
% What if the objective is to actively alter the rationale itself?

% The rationale attack is designed to proactively modify the rationale part and subsequently attack the choice letter. 
% After randomly selecting several samples from both models, we observed that the distributions are similar to that observed under the answer attack scenario (see Table \ref{tab-rat_chg}).
% %%%%%%%%%%%%%%%%% ORG %%%%%%%%%%%%%%%%%%%%%
% The section \ref{sec-ch_ana} shows that to successfully attack the model, a change in the rationale is needed in most situations.
% However, the changes in the rationale part under the answer attack scenarios are passive.
% They are changed because the answer needs to be changed.
% Then, what if the rationale is aimed to be changed?
% The rationale attack actively modifies the rationale part and attacks the choice letter.
% We randomly picked several samples on both models and found that the distribution was similar to the answer attack (Table \ref{tab-rat_chg}).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[t]
% \caption{
% Percentage of samples classified by changes in the rationale attack. The distribution of changes closely mirrors that observed under the answer attack in Table \ref{tab-ch_chg}.
% % Shown in percentage.
% % Number of samples split by the changes under the rationale attack. The changes' distribution is similar to those under the answer attack in Tabel \ref{tab-ch_chg}.
% }
% \label{tab-rat_chg}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcc}
% \toprule
% Model        & Key Changes & Trivial Changes \\
% \midrule
% MiniGPT4     & 50                              & 50                                   \\
% OpenFlamingo & 75                              & 25                                    \\
% \bottomrule
% \end{tabular}%
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{table}[]
% \centering
% \resizebox{0.8\columnwidth}{!}{%
% \begin{tabular}{lcc}
% \hline
% Model        & \multicolumn{1}{l}{Key Changes} & \multicolumn{1}{l}{Trivial Changes} \\ \hline
% MiniGPT4     & 10                              & 10                                   \\
% OpenFlamingo & 15                              & 5                                   \\ \hline
% \end{tabular}%
% }
% \caption{Number of samples split by the changes under the rationale attack. The changes' distribution is similar to those under the answer attack in Tabel \ref{tab-ch_chg}.}
% \label{tab-rat_chg}
% \end{table}

%%%%%%%%%%%%%%%%%% GPT %%%%%%%%%%%%%%%%%%%
% The two tables reveal a noteworthy conclusion: different models leverage the CoT reasoning process in distinct ways.
% In the case of OpenFlamingo, the key information within the rationale holds greater significance, and these key elements in the reasoning process contribute significantly to the observed robustness boost.
% On the contrary, for MiniGPT4, the importance of key information is less pronounced. 
% The models can produce incorrect answers even when the key information in the reasoning chain is accurate (see Figure \ref{fig-ch_trv}).
% The even distribution of changes suggests that the robustness boost is primarily contributed by the CoT reasoning process itself.
%%%%%%%%%%%%%%%%%% ORG %%%%%%%%%%%%%%%%%%%
% The two tables show an interesting conclusion: different models leverage the CoT reasoning process differently.
% For the OpenFlamingo, the key information in the rationale is more important.
% Those key parts in the reasoning process contribute to the robustness boost.
% For the MiniGPT4, the key information is not so important. 
% The models can have a wrong answer even if the key information in the reasoning chain is right (see Figure \ref{fig-ch_trv}).
% The even distribution of the changes suggest that the robustness boost is contributed by the CoT reasoning process itself.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure*}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\linewidth]{Figure/eg2.pdf}}
% \caption{Two Examples of The Three Attack Methods. 
% The figure shows two examples to compare the consequences of the three attack methods. 
% % The two examples are separated through a dotted line. 
% At the top, in both examples, it shows the callouts of a user with an input image and their associated textual questions. 
% The four callouts below are the answers from the M-LLM under each type of attacks. We can see that on the left side example, only stop-reasoning attack achieves the goal failing the model by providing a wrong answer (highlighted in red color). On the right side example, only stop-reasoning attack achieves to the goal confusing the model to conclude that there is no correct answer.
% }
% \label{fig-eg}
% \end{center}
% \vskip -0.2in
% \end{figure*}

% \subsubsection{Why is stop-reasoning attack powerful?}
% %%%%%%%%%%%%%%% GPT %%%%%%%%%%%%%%%%
% According to the experiment results presented in Section \ref{sec-quan}, the stop-reasoning attack proves to be the most powerful on MLLMs with CoT. 
% Figure \ref{fig-eg} illustrates two examples where both rationale and answer attacks fail, and only the stop-reasoning attack succeeds. 
% We were wondering What makes it so effective.

% Upon closer examination, we observe that after the stop-reasoning attack, the model outputs the answer directly without leveraging CoT, aligning with the fundamental concept of the stop-reasoning attack – aiming to halt the CoT reasoning process (see Figure \ref{fig-eg}). 
% When the stop-reasoning attack succeeds, the model disregards the prompt's CoT reasoning process requirement and directly infers the answer.

% As revealed in the analysis in Section \ref{sec:cot-rob}, the extra robustness boost is intricately tied to the generated rationale part as a byproduct from CoT reasoning process. 
% If this CoT reasoning process is unfortunately nullified, then the additional robustness generated during the CoT reasoning process will be gone as well.
% Thus, achieving the adversary's goal becomes comparatively easier.
%%%%%%%%%%%%%%% ORG %%%%%%%%%%%%%%%%
% As analyzed in section \ref{sec-quan}, the stop-reasoning attack is the most powerful on the model with CoT.
% Figure \ref{fig-eg} shows two examples. 
% The rationale and answer attacks fail in both examples.
% Only the stop-reasoning attack succeeds.
% But why is it useful?
% We observe that after the attack, the model under the stop-reasoning attack outputs the answer directly without CoT, which suits the idea of the stop-reasoning attack, i.e., the stop-reasoning attack aims to stop the CoT reasoning process (see Figure \ref{fig-eg} left).
% When the stop-reasoning attack succeeds, the model ignores the requirement of the CoT reasoning process in the prompts and infers the answer directly.
% As we suppose, the robustness boost comes from the reasoning process.
% The additional robustness boost is eliminated when the model answers the question without CoT.
% Thus, the model is more vulnerable to the attack on the answer part.
% The adversary goal is easier to achieve.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We suppose the stop-reasoning attack won't perform well for the samples that still have a rationale. 
% At least it should be worse than the answer attack.
% As introduced in section \ref{sec-stop}, the loss function of the stop-reasoning attack is built with two parts, i.e., loss on rationale part and loss on answer part.
% For a sample that can not really stop-reasoning, the 
%%%%%%%%%%%%%%%%% GPT %%%%%%%%%%%%%%%%%%
% Moreover, we found that some samples didn't really stop reasoning the model is vulnerable even if it does not completely halt its reasoning process. 
% In our exploration of these samples, we observed that with the stop-reasoning attack, even if the model still retains its reasoning ability, it is inclined to terminate its answer prematurely and can not output the answer part (see Figure \ref{fig-eg}, right).
%%%%%%%%%%%%%%%%% ORG %%%%%%%%%%%%%%%%%%
% After a further analysis, the model is vulnerable even if it does not really stop its reasoning process.
% We explored those samples and found that, with the stop-reasoning attack, even if the model still has the reasoning ability, it is prone to end its answer early and not output the answer part (see Figure \ref{fig-eg} right).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[t]
% \caption{Percentage of inferences lacking answers. 
% The table provides a summary of the proportion of samples that, despite retaining a rationale part, do not include an answer part under the stop-reasoning attack.
% % The table summarises the portion of samples that do not have an answer part when they still have a rationale part under the stop-reasoning attack.
% }
% \label{tab-null}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcc}
% \toprule
%              & A-OKVQA & ScienceQA \\ 
% \midrule
% MiniGPT4     & 96.43   & 73.58     \\
% OpenFlamingo & 62.46   & 49.25     \\ 
% \bottomrule
% \end{tabular}%
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{table}[]
% \centering
% \resizebox{0.75\columnwidth}{!}{%
% \begin{tabular}{lcc}
% \hline
%              & A-OKVQA & ScienceQA \\ 
% MiniGPT4     & 96.43   & 73.58     \\
% OpenFlamingo & 62.46   & 49.25     \\ 
% \end{tabular}%
% }
% \caption{Portion of inferences without answers. The table summarises the portion of samples that do not have an answer part when they still have a rationale part under the stop-reasoning attack.}
% \end{table}

% \begin{figure}
% \centering
% \includegraphics[width=0.95\columnwidth]{Figure/stop_ans.pdf}
% \caption{stop-reasoning attack. The two inferences share an identical instruction prompt. The inference after the stop-reasoning attack can not leverage the CoT process. The model infers the answer directly. The robustness brought by the CoT technique is then eliminated.}
% \label{fig-stop_ans}
% \end{figure}

% \begin{table}[t]
% \caption{Accuracy(\%) Table for the ImageNet Classification Task. Models correctly answer all samples when inferring with CoT and without attack. \# classes signifies the number of classes extracted from the ImageNet dataset for multi-choice classification tasks. Lower accuracy values indicate more successful attacks. Ans., Rat., and Stop. are abbreviations of answer attack, rationale attack, and stop-reasoning attack separately.
% Accuracy table of classification task on ImageNet. 
% The data are shown in percentages. 
% All the samples are correctly answered when models infer with CoT and without attack. 
% The name of the dataset indicates how many classes are extracted from the ImageNet dataset to form the multi-choice classification tasks.
% The lower the accuracy, the better the attack.
% }
% \label{tab-imagenet}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cccccc}
% \toprule
% \multicolumn{1}{c|}{\multirow{2}{*}{\# Classes}} & \multicolumn{2}{c|}{w/o CoT}                                 & \multicolumn{3}{c}{with CoT}                                                                     \\
% \multicolumn{1}{c|}{}                         & \multicolumn{1}{l}{w/o Att.} & \multicolumn{1}{l|}{Ans.} & \multicolumn{1}{l}{Ans.} & \multicolumn{1}{l}{Rat.}  & \multicolumn{1}{l}{Stop.} \\ 
% \midrule
% 4                           & 85.34                          & 0.00                       & 4.19                       & 4.71                          & \textbf{0.52}                      \\
% 8                           & 82.04                          & 0.00                       & 1.06                       & \textbf{0.00}                 & \textbf{0.00}                      \\
% 16                      & 74.32                          & 0.00                       & 3.32                       & 2.42                          & \textbf{0.30}                      \\ \bottomrule
% \end{tabular}%
% }
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}


\subsubsection{What if CoT is not necessary for tasks?}
%%%%%%%%%%%%%%%% GPT %%%%%%%%%%%%%%%%
In addition to two datasets that require reasoning, the impact on the robustness in simple classification tasks were also investigated. 
These tasks were constructed by extracting subsets from the ImageNet~\cite{russakovsky2015imagenet} dataset (see Appendix \ref{sec:cls}). 
%These classification tasks were exclusively tested on MiniGPT4 since OpenFlamingo cannot infer with CoT on those tasks.

% As depicted in Table \ref{tab-main}, the results for simple tasks align with those observed for A-OKVQA and ScienceQA datasets. i.e., CoT enhances model robustness, with the stop-reasoning attack proving the most potent against models with CoT.

% While the accuracy in the ``answer attack without CoT'' column is similar, indicating comparable robustness on models without CoT, 
A substantial gap is evident between the accuracy values of the ImageNet series and those of the A-OKVQA and ScienceQA datasets when models with CoT are under the answer attack. This discrepancy can be attributed to the inherent difficulty of VQA tasks compared to the simpler classification tasks on the ImageNet dataset.
% We hypothesize that in challenging tasks like complex VQA, the reasoning process plays a more pivotal role and brings more robustness. 
Moreover, upon further investigation of the A-OKVQA and ScienceQA datasets, we found that the A-OKVQA dataset is relatively easier. Table \ref{tab-main} illustrates an accuracy gap between the two datasets as well.
% , aligning with the hypothesis.
This performance discrepancy is observed in all three models. By comparing the accuracy of the classification task on ImageNet with the VQA tasks on A-OKVQA and ScienceQA, a significant conclusion emerges: on simple tasks that do not need a reasoning process, the CoT has almost no influence on the robustness.
%%%%%%%%%%%%%%%% ORG %%%%%%%%%%%%%%%%
% Besides the dataset that needs a reasoning process, robustness changes on simple classification tasks are also studied.
% We build simple classification tasks by extracting a subset from the ImageNet\cite{russakovsky2015imagenet} dataset.
% The classification tasks are built with four, eight, and sixteen classes separately.
% All the tasks are formulated in a multi-choice question with the classes as the choices.
% The questions to all those subsets are identical, i.e., "What is the class of the image?".
% The classification tasks were tested only on the MiniGPT4 since the OpenFlamingo can not infer with CoT on those tasks.

% As shown in Table \ref{tab-main}, the results on simple tasks are consistent with results on A-OKVQA and ScienceQA.
% The CoT reasoning process brings more robustness to the model.
% The stop-reasoning attack is the most powerful attack on the models with CoT.

% The accuracy values shown in the column answer attack without CoT are similar, which suggests the model's robustness without CoT is similar.
% However, there is a huge gap between the accuracy values of the ImageNet series and those of the A-OKVQA and ScienceQA datasets when the model with CoT is under answer attack.
% The difference between those tasks is that the VQA tasks on the A-OKVQA and the ScienceQA datasets are more difficult than the classification task on the ImageNet dataset.
% And for those difficult tasks, the reasoning process is more important.
% After further exploring the A-OKVQA and the ScienceQA datasets, we found the A-OKVQA dataset is easier, which is consistent with the accuracy performance, i.e., there is also a performance gap between the A-OKVQA dataset and the ScienceQA dataset on both MiniGPT4 and OpenFlamingo.

% By comparing the accuracy of the classification task on ImageNet and the VQA task on A-OKVQA and ScienceQA, here comes a further conclusion: the more important the CoT is, the more robustness it brings.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Perturbation Analysis}

\subsubsection{What does CoT look like when MLLMs output a wrong answer?}

In the absence of the CoT reasoning process, when MLLMs make inferences, our understanding is confined to the correctness of the answer. Delving deeper into the decision-making process and answering the question of why the model infers an unreasonable answer with an adversarial image becomes elusive.

When an MLLM is instructed to activate CoT reasoning, it opens a window into the intermediate thinking steps that models employ to derive the final answer. The rationale part generated by the CoT reasoning process provides indications and offers partial explanations on why the model infers such an unreasonable answer. We can check which key information that were attacked thus modified may ultimately lead such a wrong answer. In Figure \ref{fig:exp-smp}, we give two examples, where at the top the rationale part says that the black forehead is a distinctive black patch, which is not true, so the model incorrectly infers that that image is a panda, which is rather a money; and at the bottom the rationale part says the black and white patterns on the panda's body is the black-white picture of a bison, which is not true, so the model wrongly infers that the picture contains a bison, which is rather a panda.


% As discussed in Section \ref{sec:cot-rob}, alterations in the rationale can be classified into key changes and trivial changes. Two samples with key changes in the rationale are depicted in Figure \ref{fig:exp-smp}.
% % ; additional samples are available in Appendix \ref{sec:exp-smp}.
% On the top, a monkey is inaccurately identified as a panda, potentially influenced by the black forehead being recognized as a distinctive black patch. On the bottom, a panda is erroneously recognized as a bison, with the black and white patterns on the panda's body being interpreted as the black-white picture of a bison.
% The CoT reasoning process brings explainability to the MLLMs. MLLMs without CoT output wrong answers directly with the adversarial image. Without the reasoning process, we can not know why the model infers a wrong answer (see Figure \ref{fig-wo_chg}). The CoT reasoning process somehow reveals the inner mechanism of how the MLLMs infer a wrong answer. As illustrated in Figure \ref{fig:exp-smp},

\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figure/exp-sample_.pdf}}
\caption{CoT brings explainability to MLLMs. On the top, a monkey is falsely recognized as a panda. On the bottom, a panda is falsely recognized as a bison.}
\label{fig:exp-smp}
\end{center}
\end{figure}
